The Devil is in the Spectrum Bias: Spectrum-Balanced Feature Matching for Robust Representation Distillation

Large visual foundation models have demonstrated remarkable transferability across a wide range of downstream tasks. To deploy such models efficiently, feature matching has become a popular knowledge distillation approach that transfers teacher representations to smaller student models without requiring labeled data. However, we show that the conventional feature matching objective with L2-distance is inherently biased toward reconstructing dominant spectral directions of the teacher representation, while under-optimizing low-variance directions that often contain task-relevant information. To address this, we propose Spectrum-Balanced Feature Matching, SpecMatch, a simple objective that adaptively emphasizes under-optimized spectral directions while preserving the relative importance of dominant directions. SpecMatch is easy to implement and introduces negligible computational overhead. Extensive experiments on image recognition demonstrate that SpecMatch consistently improves downstream adaptation across diverse tasks, including image classification, anomaly detection, medical image analysis, and domain generalization. In particular, SpecMatch outperforms conventional feature matching in 40 of 42 teacher--student and training-setting combinations, while consistently improving over the original student model in all settings. We further demonstrate that the proposed objective generalizes beyond vision, improving downstream performance across six protein understanding tasks.

==> graphs/anomaly_detection_samples.tex <==
% \begin{figure}[t]
%     \centering

%     \begin{subfigure}{0.48\linewidth}
%         \centering       
%         \includegraphics[width=\linewidth]{images/anomaly_samples.png}
%         \caption{ImageNet}
%         \label{fig:imagenet}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\linewidth}
%         \centering
       
%         \caption{}
%         \label{fig:coco}
%     \end{subfigure}
%     \hfill   
%     \caption{Ours is robust in different hyper-parameters.}
%     \label{fig:samples_anomalydetection}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.4\linewidth}
        \centering   
        \vspace{0pt}        \includegraphics[width=\linewidth]{images/anomaly_samples.png}
    \end{minipage}
%    \hfill
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \small
        \vspace{4.5pt}        
       % \setlength{\tabcolsep}{4pt}
        \renewcommand{\arraystretch}{1.1}
        \begin{tabular}{lcccc}
        \toprule    
        \multirow{2}{*}{Method}
  & \multicolumn{4}{c}{iNaturalist2018}\\\cmidrule(lr){2-5}
         & Head & Medium & Tail & All \\\hline        
       % \rowcolor{blue!10} PE-Core-G14 $\rightarrow$ PE-Core-Tiny &&&&\\\hline
        PE-Core-G14 & 86.7 & 78.0 & 73.7 & 	77.2\\
        PE-Core-Tiny & 54.2 & 47.2 & 44.5 & 46.8 \\
        FM   & 60.3 & 51.8 & 51.0 & 52.3 \\
        Ours & \textbf{61.3} & \textbf{52.7} & \textbf{52.0} & \textbf{53.3} \\
        \bottomrule
        \end{tabular}
    \end{minipage}

    \caption{(a) Hyperparameter sensitivity on ImageNet. (b) Linear probing results on iNaturalist across head, medium, and tail classes.}
    \label{fig:samples_anomalydetection}
\end{figure}

==> graphs/finetuning_result.tex <==
\begin{figure}[t]
    \centering

    \begin{subfigure}{0.32\linewidth}
        \centering
        \fbox{\rule[-.5cm]{0cm}{4cm}\rule[-.5cm]{4cm}{0cm}}
        \caption{ImageNet}
        \label{fig:imagenet}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \fbox{\rule[-.5cm]{0cm}{4cm}\rule[-.5cm]{4cm}{0cm}}
        \caption{}
        \label{fig:coco}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \fbox{\rule[-.5cm]{0cm}{4cm}\rule[-.5cm]{4cm}{0cm}}
        \caption{}
        \label{fig:voc}
    \end{subfigure}

    \caption{Fine-tuning with different shots.}
    \label{fig:hyperparam}
\end{figure}

==> graphs/pca_root_change.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
           \includegraphics[width=\linewidth]{images/beta_sensitivity.png}
        \caption{ImageNet}
        \label{fig:dataset1}
    \end{subfigure}
   \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
          \includegraphics[width=\linewidth]{images/beta_sensitivity.png}
        \caption{Dataset 4}
        \label{fig:dataset4}
    \end{subfigure}
    \caption{Hyper-parameter sensitivity.}
    \label{fig:hyperparam}
\end{figure}

==> graphs/reconstruction_spectrum.tex <==
\begin{figure}[t]
    \centering
   % \includegraphics[width=0.8\linewidth]{imagenet_curve.pdf}
   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
    \caption{Teacher feature reconstruction across different spectrum.}
    \label{fig:feature_reconstruction}
\end{figure}

==> tables/effective_rank.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c c cc c c c}
\toprule
\textbf{Method}
& \textbf{ImageNet}
& \textbf{CIFAR100}
& \textbf{CUB}
& \textbf{EuroSAT}
& \textbf{OrganCMNIST}
& \textbf{Camelyon17}
& \textbf{MVTec}
\\
\midrule
Teacher
& -- & -- & -- & -- & -- & -- \\
Student
& -- & -- & -- & -- & -- & -- \\
DINO
& -- & -- & -- & -- & -- & -- \\
Vanilla FM
&  &  &  &  &  &  \\
Ours
&  &  &  &  &  &  \\
\midrule
$\Delta$ Ours -- FM
&  &  &  &  &  &  \\
\bottomrule
\end{tabular}
\caption{
Effective rank of student representations across downstream datasets.
Higher effective rank indicates a more diverse representation spectrum.
}
\label{tab:effective_rank}
\end{table*}

==> tables/hyp_l1.tex <==
% \begin{table}[t]
% \small
% \setlength{\tabcolsep}{3pt}
% \centering
% \begin{tabular}{lcccc}
% \toprule
% $\beta$ & ImageNet & Nabirds & Iwildcam & CIFAR100 \\
% \midrule
% 1 & 72.1 & 70.7 & 71.7 & 80.9 \\
% 2 & 72.7 & 73.6 & \textbf{75.0} & 82.0 \\
% 3 & \textbf{73.1} & \textbf{73.7} & 74.5 & 81.9 \\
% 4 & 72.9 & 73.4 & 73.2 & \textbf{82.3} \\
% \bottomrule
% \end{tabular}
% \hfill
% \begin{tabular}{lccccc}
% \toprule
% Method & CIFAR100 & CIFAR10 & SVHN & GTSRB & Cam17 \\
% \midrule
% Base & 76.2 & 92.1 & 57.7 & 81.5 & 89.0 \\
% L2   & 80.9 & 97.1 & 84.1 & 93.3 & \textbf{94.0} \\
% L1   & 81.2 & 97.0 & 81.7 & \textcolor{blue}{82.2} & \textcolor{blue}{81.5} \\
% Ours     & \textbf{81.9} & \textbf{97.3} & \textbf{85.8} & \textbf{94.8} & 93.4  \\
% \bottomrule
% \end{tabular}
% \vspace{-3mm}
% \caption{
% Left: Sensitivity analysis with respect to $\beta$ for distillation from PE-Core-Large to PE-Core-Tiny. $\beta=1$ corresponds to vanilla feature matching, while $\beta=2$ and $3$ consistently improve performance.
% Right: Comparison between L1 and L2 distance. In most cases, L1 loss performs on par with L2, yet L1 performs poorly in \textcolor{blue}{highlighted} cases.
% }
% \label{tab:ablation}
% \end{table}

\begin{table*}[h!]
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\centering
% Left: Sensitivity analysis
\caption{
\small
All experiments are done on distillation from PE-Core-Large to Tiny.
\textbf{\figleft:} Sensitivity analysis for $\beta$. $\beta=1$ corresponds to vanilla feature matching,
while $\beta=2$ and $3$ consistently improve performance.
\textbf{\figcenter:} Comparison between L1 and L2 distance. In most cases, L1 loss performs
on par with L2, yet L1 performs poorly in \textcolor{blue}{highlighted} cases.
\textbf{\figright:} The effect of whitening. Whitening ensures uniform loss contributions across directions; however, this does not necessarily translate into improved downstream performance.
}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
$\beta$ & ImageNet & NAB & iWild & CIF100 \\
\midrule
1 & 72.1 & 70.7 & 71.7 & 80.9 \\
2 & 72.7 & 73.6 & \textbf{75.0} & 82.0 \\
3 & \textbf{73.1} & \textbf{73.7} & 74.5 & 81.9 \\
4 & 72.9 & 73.4 & 73.2 & \textbf{82.3} \\
\bottomrule
\end{tabular}
\hspace{5mm}
%\hfill
% Middle: L1 vs. L2
\begin{tabular}{lccccc}
\toprule
Method & CIF100 & CIF10 & SVHN & GTSRB & Cam17 \\
\midrule
Base & 76.2 & 92.1 & 57.7 & 81.5 & 89.0 \\
L2   & 80.9 & 97.1 & 84.1 & 93.3 & \textbf{94.0} \\
L1   & 81.2 & 97.0 & 81.7 & \textcolor{blue}{82.2} & \textcolor{blue}{81.5} \\

\ours & \textbf{81.9} & \textbf{97.3} & \textbf{85.8} & \textbf{94.8} & 93.4 \\
\bottomrule
\end{tabular}
\hspace{5mm}

%\hfill
% Right: PE-Core-Tiny ablation
\begin{tabular}{lccc}
\toprule
Method & CUB & iWild & NAB \\
\midrule
Base        & 71.6 & 74.1 & 69.9 \\
FM          & 77.5 & 71.7 & 70.3 \\
FM + Whitening & 73.7 & 73.4 & 68.7 \\

\ours        & \textbf{79.6} & \textbf{74.5} & \textbf{73.7} \\
\bottomrule
\end{tabular}
}


\label{tab:ablation}

\end{table*}


==> tables/instance_recognition_dinov2.tex <==
\begin{table}[t]
    \centering   
    \label{tab:instance_recognition}
    \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{Method}
        & \multicolumn{3}{c}{Oxford}
        & \multicolumn{3}{c}{Paris}  & \multirow{2}{*}{Avg. Gain $\uparrow$} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        &E& M & H &E& M & H \\
        \midrule
        Teacher &87.0 & 72.2&	54.4 &94.8 & 92.4 & 83.8 & - \\
        Student & 19.7&14.7&	3.5&62.9&47.5&20.9 & -\\\arrayrulecolor{gray}
\midrule
\arrayrulecolor{black}
        DINO & 37.7 & 25.5 & 6.3 & 73.2&59.5&34.8 \\
        FM & 28.0&20.2 & 5.1&	68.8&57.6&\textbf{33.5}& 7.3\\        
        \midrule
        Ours     & 33.3 & 23.1&5.9&71.4&57.9&33.3 &9.3\\
        \bottomrule
    \end{tabular}
    \label{tab:instance_recognition}
     \caption{\small Instance recognition results on the Oxford and Paris datasets. DINOv2~\citep{oquab2023dinov2} 7B model is used as a teacher while ViT-Tiny (5.7M) is used as a student. E, M, and H denote the Easy, Medium, and Hard evaluation protocols, respectively.}
\end{table}
